Long-term collaboration with strong friendship ties improves academic performance in remote and hybrid teaching modalities in high school physics

Collaboration among students is fundamental for knowledge building and competency development. Yet, the effectiveness of student collaboration depends on the extent that these interactions occur under conditions that favor commitment, trust, and decision-making among those who interact. The sanitary situation and the transition to emergency remote teaching have added new challenges for collaboration, mainly because now, Information and Communication Technologies mediate students' interactions. This study first explores the effectiveness of different collaborative relationships on physics from a sample of secondary students from two schools located in rural and urban areas in southern Chile. We used Social Network Analysis to map students' academic prestige, collaboration, and friendship ties. We define a strong association if two students are declared mutually as friends. Using multiple linear regression models, we found positive effects of collaboration on grades, particularly among students working with friends (strong ties). Then, the second study corresponds to a quasi-experiment on four classes at the analyzed urban school during the following academic year. Here, students attended hybrid sessions to test whether the effects of collaboration found on the first study were stable throughout two semesters. Following the same procedures as in the exploratory phase, we found that the initial effects of collaboration on grades are negative for all collaborative variables, while strong working ties afford academic gains later into the year. These results contribute to the literature of collaboration in physics education and its effectiveness, taking into account social relationships and the needed time for developing beneficial collective processes among students in the classroom.

==> Table_comparative_models_Act1,2,3.tex <==
\begin{table*}[!htbp] \centering 
  \caption{} 
  \label{} 
\scriptsize 
\begin{tabular}{@{\extracolsep{5pt}}lccccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{9}{c}{\textit{Dependent variable:}} \\ 
\cline{2-10} 
\\[-1.8ex] & \multicolumn{9}{c}{Physics Grades)} \\ 
\\[-1.8ex] & (Act.1) & (Act. 2) & (Act. 3) & (Act. 1) & (Act. 2) & (Act. 3) & (Act. 1) & (Act. 2) & (Act. 3)\\ 
\hline \\[-1.8ex] 
 scale(Lam\_deg) & 0.044 & 0.029 & 0.051 & 0.032 & $-$0.048 & $-$0.328$^{**}$ & 0.029 & $-$0.010 & $-$0.180 \\ 
  & (0.119) & (0.114) & (0.109) & (0.132) & (0.158) & (0.154) & (0.127) & (0.131) & (0.135) \\ 
  & & & & & & & & & \\ 
 scale(LCF) & $-$0.300$^{***}$ & $-$0.123 & 0.067 &  &  &  &  &  &  \\ 
  & (0.102) & (0.121) & (0.105) &  &  &  &  &  &  \\ 
  & & & & & & & & & \\ 
 scale(LCFdeb) &  &  &  & $-$0.294$^{**}$ & $-$0.213$^{*}$ & $-$0.160 &  &  &  \\ 
  &  &  &  & (0.120) & (0.115) & (0.122) &  &  &  \\ 
  & & & & & & & & & \\ 
 scale(LCFfuer) &  &  &  & $-$0.256$^{*}$ & $-$0.056 & 0.393$^{**}$ &  &  &  \\ 
  &  &  &  & (0.131) & (0.166) & (0.157) &  &  &  \\ 
  & & & & & & & & & \\ 
 scale(LCFdBE) &  &  &  &  &  &  & $-$0.092 & 0.157 & 0.071 \\ 
  &  &  &  &  &  &  & (0.112) & (0.111) & (0.112) \\ 
  & & & & & & & & & \\ 
 scale(LCFfBE) &  &  &  &  &  &  & $-$0.215 & 0.190 & 0.464$^{***}$ \\ 
  &  &  &  &  &  &  & (0.145) & (0.145) & (0.128) \\ 
  & & & & & & & & & \\ 
 Group\_Friends1 & $-$0.129 & $-$0.145 & $-$0.046 & $-$0.264 & $-$0.193 & $-$0.168 & $-$0.186 & 0.163 & $-$0.114 \\ 
  & (0.203) & (0.243) & (0.202) & (0.228) & (0.242) & (0.201) & (0.224) & (0.236) & (0.202) \\ 
  & & & & & & & & & \\ 
 GeneroM & 0.457$^{*}$ & $-$0.750$^{***}$ & $-$0.613$^{***}$ & 0.472$^{*}$ & $-$0.783$^{***}$ & $-$0.518$^{**}$ & 0.540$^{**}$ & $-$0.658$^{***}$ & $-$0.470$^{**}$ \\ 
  & (0.236) & (0.229) & (0.222) & (0.238) & (0.229) & (0.214) & (0.244) & (0.227) & (0.212) \\ 
  & & & & & & & & & \\ 
 scale(LPhys) & 0.009 & $-$0.009 & 0.205$^{*}$ & 0.033 & $-$0.039 & 0.193$^{*}$ & 0.068 & $-$0.031 & 0.076 \\ 
  & (0.124) & (0.120) & (0.116) & (0.124) & (0.121) & (0.110) & (0.129) & (0.120) & (0.115) \\ 
  & & & & & & & & & \\ 
 scale(lbe\_ind) & 0.294$^{**}$ & 0.168 & $-$0.063 & 0.307$^{**}$ & 0.165 & $-$0.057 & 0.396$^{**}$ & 0.057 & $-$0.132 \\ 
  & (0.132) & (0.129) & (0.111) & (0.138) & (0.129) & (0.103) & (0.159) & (0.138) & (0.104) \\ 
  & & & & & & & & & \\ 
 Constant & $-$0.148 & 0.424$^{**}$ & 0.310$^{*}$ & $-$0.085 & 0.464$^{**}$ & 0.327$^{*}$ & $-$0.157 & 0.223 & 0.278 \\ 
  & (0.185) & (0.187) & (0.178) & (0.197) & (0.186) & (0.174) & (0.196) & (0.183) & (0.174) \\ 
  & & & & & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 90 & 90 & 90 & 90 & 90 & 90 & 90 & 90 & 90 \\ 
R$^{2}$ & 0.193 & 0.203 & 0.216 & 0.194 & 0.225 & 0.315 & 0.137 & 0.230 & 0.330 \\ 
Adjusted R$^{2}$ & 0.134 & 0.145 & 0.159 & 0.125 & 0.159 & 0.256 & 0.063 & 0.164 & 0.273 \\ 
Residual Std. Error & 0.930 (df = 83) & 0.925 (df = 83) & 0.917 (df = 83) & 0.936 (df = 82) & 0.917 (df = 82) & 0.862 (df = 82) & 0.968 (df = 82) & 0.914 (df = 82) & 0.852 (df = 82) \\ 
F Statistic & 3.300$^{***}$ (df = 6; 83) & 3.514$^{***}$ (df = 6; 83) & 3.814$^{***}$ (df = 6; 83) & 2.811$^{**}$ (df = 7; 82) & 3.407$^{***}$ (df = 7; 82) & 5.384$^{***}$ (df = 7; 82) & 1.861$^{*}$ (df = 7; 82) & 3.491$^{***}$ (df = 7; 82) & 5.781$^{***}$ (df = 7; 82) \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{9}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table*}

==> did_table.tex <==
\begin{table*}[!htbp] \centering 
  \caption{} 
  \label{} 
\scriptsize 
\begin{tabular}{@{\extracolsep{5pt}}lcccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{6}{c}{\textit{Dependent variable:}} \\ 
\cline{2-7} 
\\[-1.8ex] & \multicolumn{6}{c}{scale(lnota)} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6)\\ 
\hline \\[-1.8ex] 
 GeneroM & $-$0.032 & 0.046 & $-$0.032 & 0.071 & 0.008 & $-$0.029 \\ 
  & (0.154) & (0.148) & (0.148) & (0.148) & (0.155) & (0.145) \\ 
  & & & & & & \\ 
 Random\_Friends1 & 0.212 & 0.147 & 0.335$^{**}$ & 0.141 & 0.139 & 0.349$^{**}$ \\ 
  & (0.149) & (0.149) & (0.154) & (0.148) & (0.156) & (0.153) \\ 
  & & & & & & \\ 
 Act311 & 0.317$^{**}$ & 0.353$^{**}$ & 0.282$^{*}$ & 0.350$^{**}$ & 0.305$^{**}$ & 0.297$^{**}$ \\ 
  & (0.150) & (0.150) & (0.148) & (0.148) & (0.152) & (0.146) \\ 
  & & & & & & \\ 
 scale(LCF) & $-$0.257$^{***}$ &  &  &  &  &  \\ 
  & (0.095) &  &  &  &  &  \\ 
  & & & & & & \\ 
 scale(LCFdeb) &  &  & $-$0.409$^{***}$ &  &  & $-$0.438$^{***}$ \\ 
  &  &  & (0.118) &  &  & (0.118) \\ 
  & & & & & & \\ 
 scale(LCFdBE) &  &  &  &  & $-$0.049 &  \\ 
  &  &  &  &  & (0.108) &  \\ 
  & & & & & & \\ 
 scale(Lam\_deg) & 0.132 &  & 0.017 &  & 0.144$^{*}$ &  \\ 
  & (0.083) &  & (0.087) &  & (0.081) &  \\ 
  & & & & & & \\ 
 scale(BE1\_ind) & 0.056 &  &  &  &  &  \\ 
  & (0.078) &  &  &  &  &  \\ 
  & & & & & & \\ 
 Act311:scale(LCF) & 0.277$^{*}$ &  &  &  &  &  \\ 
  & (0.152) &  &  &  &  &  \\ 
  & & & & & & \\ 
 scale(LCFfuer) &  & 0.020 &  &  &  & $-$0.049 \\ 
  &  & (0.101) &  &  &  & (0.082) \\ 
  & & & & & & \\ 
 Act311:scale(LCFfuer) &  & 0.099 &  &  &  &  \\ 
  &  & (0.152) &  &  &  &  \\ 
  & & & & & & \\ 
 Act311:scale(LCFdeb) &  &  & 0.297$^{**}$ &  &  & 0.291$^{**}$ \\ 
  &  &  & (0.146) &  &  & (0.146) \\ 
  & & & & & & \\ 
 scale(LCFfBE) &  &  &  & 0.074 &  &  \\ 
  &  &  &  & (0.101) &  &  \\ 
  & & & & & & \\ 
 Act311:scale(LCFfBE) &  &  &  & 0.106 &  &  \\ 
  &  &  &  & (0.149) &  &  \\ 
  & & & & & & \\ 
 Act311:scale(LCFdBE) &  &  &  &  & 0.166 &  \\ 
  &  &  &  &  & (0.150) &  \\ 
  & & & & & & \\ 
 Constant & $-$0.258$^{*}$ & $-$0.279$^{*}$ & $-$0.265$^{*}$ & $-$0.283$^{*}$ & $-$0.225 & $-$0.281$^{*}$ \\ 
  & (0.149) & (0.148) & (0.148) & (0.147) & (0.151) & (0.143) \\ 
  & & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 180 & 180 & 180 & 180 & 180 & 180 \\ 
R$^{2}$ & 0.095 & 0.048 & 0.117 & 0.059 & 0.063 & 0.118 \\ 
Adjusted R$^{2}$ & 0.058 & 0.021 & 0.086 & 0.032 & 0.030 & 0.088 \\ 
Residual Std. Error & 0.970 (df = 172) & 0.990 (df = 174) & 0.956 (df = 173) & 0.984 (df = 174) & 0.985 (df = 173) & 0.955 (df = 173) \\ 
F Statistic & 2.586$^{**}$ (df = 7; 172) & 1.751 (df = 5; 174) & 3.813$^{***}$ (df = 6; 173) & 2.188$^{*}$ (df = 5; 174) & 1.924$^{*}$ (df = 6; 173) & 3.874$^{***}$ (df = 6; 173) \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{6}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table*}

